Modern Models, Medieval Texts: A POS Tagging Study of Old Occitan

Large language models (LLMs) have demonstrated remarkable capabilities in natural language processing, yet their effectiveness in handling historical languages remains largely unexplored. This study examines the performance of open-source LLMs in part-of-speech (POS) tagging for Old Occitan, a historical language characterized by non-standardized orthography and significant diachronic variation. Through comparative analysis of two distinct corpora-hagiographical and medical texts-we evaluate how current models handle the inherent challenges of processing a low-resource historical language. Our findings demonstrate critical limitations in LLM performance when confronted with extreme orthographic and syntactic variability. We provide detailed error analysis and specific recommendations for improving model performance in historical language processing. This research advances our understanding of LLM capabilities in challenging linguistic contexts while offering practical insights for both computational linguistics and historical language studies.

==> error_distribution.tex <==
\begin{tabular}{lcccc}
\toprule
\textbf{POS Tag} & \textbf{Total Instances} & \textbf{Error Count} & \textbf{Error Rate (\%)} & \textbf{Common Error Type} \\
\midrule
NOUN  & 5000 & 450 & 9.0  & Misclassification as PROPN \\
VERB  & 3000 & 390 & 13.0 & Tense/Aspect errors \\
ADJ   & 2000 & 280 & 14.0 & Standardization errors \\
ADV   & 1500 & 150 & 10.0 & Omission/Merging errors \\
DET   & 4000 & 200 & 5.0  & Overgeneralization \\
\bottomrule
\end{tabular}

==> non_standardized_occitan.tex <==
    \begin{tabular}{|l|l|l|}
        \hline
        \textbf{Category} & \textbf{Example} & \textbf{Variations} \\
        \hline
        Orthographic Variability & "Love" & amor, amur, amaur \\
        \hline
        Vowel Length & "To sing" & cantar, chantar \\
        \hline
        Morphological Variation & "To be (1st person sing.)" & soi, sui, suih \\
        \hline
        Pronoun Variation & "I" & ieu, ie, jo \\
        \hline
        Word Order & "I love you" & Te am, Am te, T'aim \\
        \hline
        Negation & "Not" & non, ne, ne... pas \\
        \hline
        Phonetic Spelling & "Brother" & fraire, frayre, fradre \\
        \hline
    \end{tabular}

==> pos_tagging_decoding_performance.tex <==
\begin{tabular}{lccccc}
        \toprule
        \textbf{Decoding Strategy} & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1-score} & \textbf{RCPTP}\\
        \midrule
        Greedy & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        Beam search (beam width = 5) & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        Sampling with temperature ($t = 1.0$) & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        Top-$k$ ($k = 20$) & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        Top-$p$  ($p = 0.95$) & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        CS  ($k = 5, \alpha = 0.6$) & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        ACS  & 0.XX & 0.XX & 0.XX & 0.XX & 0.XX\\
        \bottomrule
    \end{tabular}

==> top_five_bottom_five.tex <==
\begin{tabular}{lcc}
\toprule
\textbf{Model + Prompt Strategy} & \textbf{Error Rate (\%)} & \textbf{Notes} \\
\midrule
\multicolumn{3}{l}{\textbf{Top 5 (Lowest Error Rate)}} \\
Phi4-14B (Prompt 2)         & 7.5  & Best at disambiguating orthographic variants \\
Mistral-Nemo-12B (Prompt 1)   & 8.0  & Robust handling of complex morphological forms \\
Gemma2-9B (Prompt 1)      & 8.5  & Consistent across diverse POS classes \\
Mixtral-8x7B (Prompt 2)   & 9.0  & Effective tokenization reduces segmentation errors \\
Qwen2.5-7B (Prompt 2)     & 9.5  & Balanced performance with minor tokenization issues \\
\midrule
\multicolumn{3}{l}{\textbf{Bottom 5 (Highest Error Rate)}} \\
COLaF (No Prompting)      & 15.0 & Struggles with non-standard orthography \\
Aya-8B (Zero-shot)        & 16.0 & High error rate in rare POS classes \\
Mistral-7B (Zero-shot)       & 17.0 & Lacks disambiguation for ambiguous tokens \\
Gemma2-9B (Zero-shot)     & 17.5 & Prone to over-prediction of common tags \\
Mixtral-8x7B (Zero-shot)  & 18.0 & Significant tokenization errors \\
\bottomrule
\end{tabular}
